Sampling in Software Engineering Research: A Critical Review and Guidelines

Representative sampling appears rare in empirical software engineering research. Not all studies need representative samples, but a general lack of representative sampling undermines a scientific field. This article therefore reports a critical review of the state of sampling in recent, high-quality software engineering research. The key findings are: (1) random sampling is rare; (2) sophisticated sampling strategies are very rare; (3) sampling, representativeness and randomness often appear misunderstood. These findings suggest that software engineering research has a generalizability crisis. To address these problems, this paper synthesizes existing knowledge of sampling into a succinct primer and proposes extensive guidelines for improving the conduct, presentation and evaluation of sampling in software engineering research. It is further recommended that while researchers should strive for more representative samples, disparaging non-probability sampling is generally capricious and particularly misguided for predominately qualitative research.

==> tables/papers.tex <==
\begin{table*}
\caption{Number of ESEM papers in each year \label{tab_papers}}
\begin{tabular*}{\linewidth}{p{0.1\linewidth}p{0.1\linewidth}p{0.4\linewidth}p{0.32\linewidth}}
%\begin{tabular*}{cccc}
\toprule
Year & Paper count \\
\midrule        
2016 & 51 \\
2015 & 36 \\
2014 & 60 \\
2013 & 48 \\
2012 & 41 \\
\bottomrule   
\end{tabular*}
\end{table*}


==> tables/sampling-method.tex <==
\begin{table*}
\caption{Sampling techniques by research methodology\label{tab_STRS}}
\centering
\begin{tabular}{lrrrrrrrrrr|r}
\par
\toprule
Research methodology & PS & CS & TSS & SS & SBS & HS & STS  & QS & SYS  & ES & total\\
\midrule        
Case study & 52 & 7 & 6 & 0 & 0 & 2 &  0 & 0 & 0 & 1 & 68 \\
Quasi-experiment & 25 & 9 & 0 & 3 & 0 & 1 & 0 & 1 & 1 & 0 & 40 \\
Experiment & 16 & 19 & 0 & 3 & 0 & 0 & 1 & 0 & 0 & 0 & 39 \\
Literature review & 9 & 2 & 2 & 3 & 5 & 0 & 0 & 0 & 0 & 0 & 21 \\
Questionnaire & 7 & 8 & 2 & 0 & 0 & 1 & 1 & 0 & 0 & 0 & 19\\
Quantitative data analysis & 16 & 2 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 18\\
Interview & 14 & 1 & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 16 \\
Mixed method & 5 & 4 & 4 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 13 \\
Grounded Theory & 0 & 1 & 0 & 0 & 0 & 0 &  0 & 0 & 0 & 0 & 1 \\
Action Research & 1 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 1 \\
\bottomrule   
\end{tabular}
\end{table*}

==> tables/sampling-year.tex <==
\begin{table}
\caption{Sampling Methods by Year \label{tab_STCY}}
\centering
\begin{tabular}{cccccc}
\par
\toprule
Method & 2012 & 2013 & 2014 & 2015 & 2016 \\
\midrule        
PS & 30 & 31 & 32 & 22 & 30 \\
CS & 8 & 12 & 16 & 7 & 10 \\
TSS & 1 & 3 & 5 & 2 & 4 \\
SS  & 2 & 2 & 1 & 2 & 2 \\
SBS & 0 & 0 & 4 & 1 & 0 \\
HS & 0 & 0 & 0 & 0 & 4 \\
STS & 0 & 0 & 1 & 1 & 0 \\
ES & 0 & 0 & 0 & 0 & 1 \\
QS & 0 & 0 & 0 & 1 & 0 \\
SYS & 0 & 0 & 1 & 0 & 0 \\
\midrule
Total & 41 & 48 & 60 & 36 & 51 \\
\bottomrule   
\end{tabular}
\end{table}

==> tables/samplingYearSummary.tex <==
\begin{table*}
\caption{Sampling techniques over the years \label{tab_ST}}
\centering
\begin{tabular}{lccccc}
\par
\toprule
Year & 2016 & 2015 & 2014 & 2013 & 2012 \\
\midrule        
Purposive Sampling & 58.82 & 61.11 & 51.66 & 62.5 & 73.17 \\
Convenience Sampling & 19.6 & 19.44 & 25 & 25 & 19.51 \\
Two stage sampling & 5.88 & 5.55 & 6.66 & 6.25 & 2.43 \\
\bottomrule   
\end{tabular}
\end{table*}
